InfTDA: A Simple TopDown Mechanism for Hierarchical Differentially Private Counting Queries

This paper extends $\texttt{InfTDA}$, a mechanism proposed in (Boninsegna, Silvestri, PETS 2025) for mobility datasets with origin and destination trips, in a general setting. The algorithm presented in this paper works for any dataset of $d$ categorical features and produces a differentially private synthetic dataset that answers all hierarchical queries, a special case of marginals, each with bounded maximum absolute error. The algorithm builds upon the TopDown mechanism developed for the 2020 US Census.

==> pseudocodes/InfTDA.tex <==
\begin{algorithm}[t]
\caption{\texttt{InfTDA}}
\begin{algorithmic}[1]
\Require Tree $\mathcal{T}=(V,E)$ of depth $T$, privacy budget $\rho>0$.
\State $\tilde{V}_0\gets \{(u_0, n)\}$
\For{$\ell \in (1,\dots, T)$} 
    \State $\tilde{V}_\ell \gets \{\}$ 
    \For {$(u, c) \in \tilde{V}_{\ell-1}$} 
        \vspace{2pt}
        \State $\tilde{\bf q} \gets {\bf q}_{\mathcal{C}}(u)+\mathcal{N}_{\mathbb{Z}}\big(0,T/\rho\big)^{\dim({{\bf q}_{\mathcal{C}}(u)})}$
        \vspace{2pt}
        \State $\bar{\bf q} \gets \texttt{IntOpt$_\infty$}\big(\tilde{\bf q}\,,\, c\big)$ 
        \vspace{2pt}
        \State $C \gets \mathcal{C}(u)$ \Comment{Collect set of child nodes of $u$}
        \State $X \gets \{(C_j, \bar{q}_j)\,:\, \bar{q}_{j}>0\}$ 
        \State $\tilde{V}_{\ell} \gets \tilde{V}_{\ell} \cup X$ 
    \EndFor
\EndFor\\
\Return $\tilde{\mathcal{T}} \gets \big(\cup_{\ell=0}^{T}\tilde{V}_\ell, E\big)$
\end{algorithmic}
\end{algorithm}

==> pseudocodes/IntOPT.tex <==
\begin{algorithm}[t]
	\caption{ Polynomial time $\ell_\infty$ Integer Optimization (\texttt{IntOpt$_\infty$})}\label{algo: Fast IntOpt}
	\begin{algorithmic}[1]
		\Require ${\bf x} \in \mathbb{Z}^b, c\in \mathbb{N}$.
		\State ${\bf z} \gets \max\big(\big\lceil \frac{c-\sum_{i}x_i}{b}\big\rceil , -{\bf x}\big)$
        \State $t \gets ||\bf{z}||_{\infty}$
        \State $I \gets \text{sorted indices of ${\bf x}$}$
        \State $I \gets (i\in I : z_i > -x_i)$
        \State $j\gets 0$
        \While{$\sum_i z_i > c-\sum_i{x_i}$}
            \State $\Delta \gets \sum_i z_i - c+\sum_i x_i$
            \State $z_{I[j]} \gets \max(z_{I[j]}-\Delta, -x_{I[j]}, -t)$
            \State $j \gets (j + 1) \mod |I|$
            \If {$j = 0$}
                \State $I \gets (i\in I : z_i > -x_i)$
                \State $r \gets \big \lfloor \frac{1}{|I|}\big(\sum_{i}z_i -c + \sum_{i}x_i\big) \big\rfloor$
                \State $t \gets t + \max(1, r)$
            \EndIf
        \EndWhile
        \State \bf{return } ${\bf x}+ {\bf z}$
	\end{algorithmic}
\end{algorithm}
